Testing (Conditional) Mutual Information

We investigate the sample complexity of mutual information and conditional mutual information testing. For conditional mutual information testing, given access to independent samples of a triple of random variables $(A, B, C)$ with unknown distribution, we want to distinguish between two cases: (i) $A$ and $C$ are conditionally independent, i.e., $I(A\!:\!C|B) = 0$, and (ii) $A$ and $C$ are conditionally dependent, i.e., $I(A\!:\!C|B) \geq \varepsilon$ for some threshold $\varepsilon$. We establish an upper bound on the number of samples required to distinguish between the two cases with high confidence, as a function of $\varepsilon$ and the three alphabet sizes. We conjecture that our bound is tight and show that this is indeed the case in several parameter regimes. For the special case of mutual information testing (when $B$ is trivial), we establish the necessary and sufficient number of samples required up to polylogarithmic terms. Our technical contributions include a novel method to efficiently simulate weakly correlated samples from the conditionally independent distribution $P_{A|B} P_{C|B} P_B$ given access to samples from an unknown distribution $P_{ABC}$, and a new estimator for equivalence testing that can handle such correlated samples, which might be of independent interest.

==> cmi_upper.tex <==
\section{Conditional Mutual Information Testing}

To do:

1. write in terms of queue instead of bins

2. check sampling with/without replacement (probably resolved with 1?)

3. samples in bins are not misclassified

4. we dont sample from $q$, but a slightly modified $\tilde q$: we need to apply the same technique to $p$, resulting in $\tilde p$, such that $p=q$ implies $\tilde p=\tilde q$ (as $p=q$ does not mean $p=\tilde q$!)

5. when going from $p_b$ to $\tilde p_b$: we need to argue that whp, no $b$ collides more than $c$ times.

6. $|p[S]|$ or $\tilde p[S]$

7. Scaling in $A$ and $C$ may not be tight

8. Double check large eigenvalues

\begin{theorem}
Let $p$ and $q$ be two unknown distributions defined over $[n]$, and $\eps \in (0,1)$ be a proximity parameter. Given sample access to $p$ and $q$, in order to distinguish between $p=q$ and $H^2(p,q) \geq \eps$ with probability at least $2/3$, $\widetilde{O}\left(\min\{\frac{n^{2/3}}{\eps^{4/3}}, \frac{n^{3/4}}{\eps}\}\right)$ samples from $p$ and $q$ are sufficient.
\end{theorem}


\subsection{Reduction to Squared Hellinger Distance Testing}
Robustness, and 
\begin{equation}
    D(p\|q)\leq O(\log(1/q_{\min}))D_H^2(p\|q)
\end{equation}

\subsection{Squared Hellinger Distance Testing wrt Petz}
The underlying idea is to perform equivalence testing between $p_{ABC}$ and $\petz_p(p)=p_{AB}p_{BC}/p_B$, which requires us to be able to sample from $\petz_p(p)$. As we will see, sampling from the latter is difficult if there is a $b$ with $p_b$ small, which is why we will need to modify our sampling: there will a small regime, the $b$'s are grouped together in $S$, and a large regime, denoted by $L$. In total we will take $N=O(\max\{N_L,N_S\})$ samples, where $N_S$ and $N_L$ denote the number of samples we need to solve the problem in the respective regime, which is divided by a threshold $p_{th}=O(1/N_S)$. We can determine with high probability to determine for each $b$ into which category it belongs, and then group the samples accordingly. We then perform the equivalence testing for both regions to precision $\epsilon/2$ each, using different techniques: 
\begin{itemize}
    \item For comparing $p[L]$ and $\petz(p)[L]$, we will need $N_L$ samples of both distributions, which we create as follows: we first take $\tilde O(N)$ of the $N$ samples which we sort into queues dependent on their $b$-value, all $b\in S$ are collected in the same queue. We then take $N$ more samples. If a sample $(a,b,c)$ appears, we keep $(a,b)$, and take a second sample by removing an element from the $b$-bin, resulting in $(a',b,c')$. We then return $(a,b,c')$. The probability to see $(a,b,c')$ is $p_{ab}$ times the probability to draw $c'$ from the $b$-queue, which is $p_{bc'}/p_b$, resulting in 
    \begin{equation}
        \Pr[(a,b,c')]=\frac{p_{ab}p_{bc'}}{p_b},
    \end{equation}
    as required. The issue with this technique arises when $p_b$ is so small that we cannot guarantee that the corresponding queue will contain enough samples to give an output. Since the values are in $L$, we can guarantee that there are always enough samples in the bin to form a sample.
    \item For the regime of small eigenvalues, we take a different approach. In fact, we modify the sampling here as follows: we require $O(N_S)$ samples. When taking the additional samples, and a small element appears, we will not pick a suitable partner. Instead, we pick any rare pair. This will distort the distribution a bit, which enforces us to modify the sampling: in the end we do equivalence testing between $\tilde p[S]$ and $\tilde\petz(p)[S]$ with a threshold $\tilde \epsilon$, with $\tilde \epsilon$ chosen such that this test implies the answer to whether $p=\petz(p)$ or $D_H^2(p,\petz(p))\geq \epsilon/2$.
\end{itemize}
{\color{red}I think we invest the same amount of samples for both regimes?}
If we take $O(N\log(N))$ samples, and assume the sample complexity scales at least with $d_B^{1/2}$ (or any other small constant), the cutoff will be at $1/N$: using Chernoff and $\mu=O(\log(N))$, 
\begin{equation}
    \Pr[|X-\mu|\geq \delta\mu]\leq 2e^{-\delta^2\mu/2}\implies \Pr[|X-\mu|\geq \mu/2]\leq 2e^{-O(\log(d_B))/8}\leq O\left(\frac{1}{d_B}\right),
\end{equation}
and a union bound guarantees that with high probability, we have $X_i$ up to a factor of $2$ within the expected value: this allows us to pick the first step a factor $2$ more samples to ensure that we have enough samples to form pairs.
{\color{red}Here we will get problems with dependencies: is the Poissonization trick enough?}
Since the smaller eigenvalues will dictate the choice of the cut-off, we start with this regime.


\subsubsection{Small eigenvalues}
Before we start with the formal part, we want to give some intuition for the sample complexity. [Give the back of the envelope argument which gives the correct scaling]


For simplicity, we write $x_{abc}:=Mp_{abc}=Mp_{ac|b}p_b$ in the following, and often leave out the index $abc$, if it is clear from the context. $X_{abc}$ denotes how often $abc$ appeared, and $x_{abc}$ is the expectation value. Denote by $\tilde X_b$ the number of $(a,c)$ pairs with $b$, $\tilde X_b=\sum_{a,c}X_{abc}$.
We have: 
\begin{align}
    \Pr[X_{abc}=k]&=\sum_{l=k}^{\infty}\Pr[X_{abc}=k|X_b=l]\Pr[X_b=l]
    \\
    &=\sum_{l=k}^{\infty}\binom{l}{k}p_{ac|b}^l(1-p_{ac|b})^{k-l}\left(\frac{x_{b}^{2l}e^{-x_{b}}}{(2l)!}+\frac{x_{b}^{2l+1}e^{-x_{b}}}{(2l+1)!}\right),
    \label{eq:cmi_smallpb_distribution}
\end{align}

\begin{lemma}
For $X_{abc}$ distributed according to \eqref{eq:cmi_smallpb_distribution}, it holds that {\color{red}TODO: upper bound}
\begin{align}
    \E[X_{abc}]&=p_{ac|b}\E[X_{b}]=p_{ac|b}\left[\frac{Mp_{b}}{2}-\frac{e^{-Mp_{b}}}{2}\sinh(Mp_{b})\right],\\\E[X_{abc}^2]&=p_{ac|b}\E[X_{b}^2]=p_{ac|b}\left[\frac{M^2p_{b}^2}{4}-\frac{Mp_{b}e^{-2Mp_{b}}}{4}+\frac{e^{-Mp_{b}}}{4}\sinh(Mp_{b})\right],
    \\
    \E[X_{abc}X_{a'bc'}]&\leq p_{ac|b}p_{a'c'|b}M^3p_b^3
\end{align}
Note that while we require $(a,c)\neq (a,c)$, $a=a'$ or $c=c'$ is allowed.
\end{lemma}
\begin{proof}
    \begin{align}
    \E[X_{abc}]&=\sum_{k=0}^{\infty}\sum_{l=k}^{\infty}k\Pr[X_{abc}=k|X_b=l]\Pr[X_b=l]
    \\
    &=\sum_{k=0}^{\infty}\sum_{l=0}^{\infty}k\Pr[X_{abc}=k|X_b=l]\Pr[X_b=l]
    \\
    &=\sum_{l=0}^{\infty}\sum_{k=0}^{\infty}k\Pr[X_{abc}=k|X_b=l]\Pr[X_b=l]
    \\
    &=\sum_{l=0}^{\infty}\sum_{k=0}^{l}k\Pr[X_{abc}=k|X_b=l]\Pr[X_b=l]
    \\
    &=\sum_{l=0}^{\infty}\left[\sum_{k=0}^{l}k\binom{l}{k}p_{ac|b}^l(1-p_{ac|b})^{k-l}\right]\left(\frac{x_{b}^{2l}e^{-x_{b}}}{(2l)!}+\frac{x_{b}^{2l+1}e^{-x_{b}}}{(2l+1)!}\right)
    \\
    &=\sum_{l=0}^{\infty}lp_{ac|b}\left(\frac{x_{b}^{2l}e^{-x_{b}}}{(2l)!}+\frac{x_{b}^{2l+1}e^{-x_{b}}}{(2l+1)!}\right)=p_{ac|b}\E[X_b].
\end{align}
Analogously, $\E[X_{abc}^2]=p_{ac|b}\E[X_b^2]$

In the following steps, we neglect the inidices $abc$ for simplicity.
\begin{align}
    \sum_{k=0}^{\infty}k\frac{x^{2k}e^{-x}}{(2k)!}&=\frac{x}{2}\sum_{k=1}^{\infty}\frac{x^{2k-1}e^{-x}}{(2k-1)!}=\frac{x}{2}\sum_{k=0}^{\infty}\frac{x^{2k+1}e^{-x}}{(2k+1)!}=\frac{xe^{-x}}{2}\sinh(x)
    \\
    \sum_{k=0}^{\infty}k\frac{x^{2k+1}e^{-x}}{(2k+1)!}&=\frac{1}{2}\sum_{k=0}^{\infty}(2k+1)\frac{x^{2k+1}e^{-x}}{(2k+1)!}-\frac{1}{2}\frac{x^{2k+1}e^{-x}}{(2k+1)!}=\frac{e^{-x}}{2}\left[x\cosh(x)-\sinh(x)\right]
    \\
    \sum_{k=0}^{\infty}k^2\frac{x^{2k}e^{-x}}{(2k)!}&=\sum_{k=0}^{\infty}\left[\frac{(2k)(2k-1)}{4}+\frac{k}{2}\right]\frac{x^{2k}e^{-x}}{(2k)!}=\frac{e^{-x}}{4}\left[x^2\cosh(x)+x\sinh(x)\right]
    \\
    \sum_{k=0}^{\infty}k^2\frac{x^{2k+1}e^{-x}}{(2k+1)!}&=\sum_{k=0}^{\infty}\left[\frac{(2k)(2k+1)}{4}-\frac{k}{2}\right]\frac{x^{2k+1}e^{-x}}{(2k+1)!}
    =\frac{e^{-x}}{4}\left[x^2\sinh(x)-x\cosh(x)+\sinh(x)\right]
\end{align}
This allows us to calculate:
\begin{align}
    \E[X_{abc}]&=p_{ac|b}\left[\frac{x_{b}}{2}-\frac{e^{-x_{b}}}{2}\sinh(x_{b})\right],\quad \quad \E[X_{abc}^2]=p_{ac|b}\left[\frac{x_{b}^2}{4}-\frac{x_{b}e^{-2x_{b}}}{4}+\frac{e^{-x_{b}}}{4}\sinh(x_{b})\right].
\end{align}
To bound this further, note that 
\begin{align}
    \E[X_b^2]&=\frac{2x_b^2+1}{8}-\frac{2x_b+1}{8}e^{-2x_b}
    \leq \frac{2x_b^2+1}{8}-\frac{(1+2x_b)(1-2x_b)}{8}=\frac{3}{4}x_b^2
\end{align}
In the following, assume $(a,c)\neq (a',c')$, but $a=a'$ or $c=c'$ is permitted. For $0<x,y$ with $x+y<1$ such that $(1-x-y)^z\leq (1-x-y+xy)^z=(1-x)^z(1-y)^z$. Then
\begin{align}
\E[X_{abc}X_{a'bc'}]
&=\sum_{k,l,s=0}kl\Pr[X_{abc}=k,X_{abc'}=l|X_b=s]\Pr[X_b=s]
\\
&=\sum_{s=0}^{\infty}\left[\sum_{k=0}^{s}\sum_{l=0}^{s-k}kl\binom{s}{k}\binom{s-k}{l}p_{ac|b}^lp_{a'c'|b}^k(1-p_{ac|b}-p_{a'c'|b})^{s-k-l}\right]\Pr[X_b=s]
\\
&=\sum_{s=2}^{\infty}\left[\sum_{k=1}^{s}\sum_{l=1}^{s-k}kl\binom{s}{k}\binom{s-k}{l}p_{ac|b}^lp_{a'c'|b}^k(1-p_{ac|b}-p_{a'c'|b})^{s-k-l}\right]\Pr[X_b=s]
\\
&\leq\sum_{s=2}^{\infty}\left[\sum_{k=1}^{s}k\binom{s}{k}p_{a'c'|b}^k(1-p_{a'c'|b})^{s-k}\sum_{l=1}^{s-k}l\binom{s-k}{l}p_{ac|b}^l(1-p_{ac|b})^{s-k-l}\right]\Pr[X_b=s]
\\
&\leq p_{ac|b}p_{a'c'|b}\sum_{s=2}^{\infty}\left[\sum_{k=1}^{s}\binom{s-1}{k-1}s(s-k)p_{a'c'|b}^{k-1}(1-p_{a'c'|b})^{s-k}\right]\Pr[X_b=s]
\\
&\leq 
p_{ac|b}p_{a'c'|b}\sum_{s=2}^{\infty}s^2\left(\frac{x_{b}^{2s}e^{-x_{b}}}{(2s)!}+\frac{x_{b}^{2s+1}e^{-x_{b}}}{(2s+1)!}\right)
\\
&\leq p_{ac|b}p_{a'c'|b}(\E[X_b^2]-(x_b^2e^{-x_b}/2+x_b^{3}e^{-x_b}/6))
\\
&= p_{ac|b}p_{a'c'|b}\left(\frac{2x_b^2+1}{8}-\frac{2x_b+1}{8}e^{-2x
_b}-\left(\frac{x_b^2e^{-x_b}}{2}+\frac{x_b^{3}e^{-x_b}}{6}\right)\right)
\end{align}
where we made use of $e^{-x}\geq 1-x+x^2/4$ in the end.
\end{proof}
We will use the following estimator:

\begin{lemma}
    \begin{equation}
        \Var[Z]\leq O(\|p[S]\|_2^2M^2)
    \end{equation}
\end{lemma}
\begin{proof}
    \begin{align}
    Z_i^2&=X_i^2(X_i')^2+4X_i^2Y_i^2+Y_i^2(Y_i')^2-4X_i^2X_i'Y_i+2X_iX_i'Y_iY_i'-4X_iY_i^2Y_i'
    \\
    \E[Z_i^2]&=\E[X_i^2]^2+4\E[X_i^2]\E[Y_i^2]+\E[Y_i^2]^2-4\E[X_i^2]\E[X_i]\E[Y_i]+2\E[X_i]^2\E[Y_i]^2-4\E[X_i]\E[Y_i^2]\E[Y_i]
    \\
    \E[Z_i]^2&=\E[X_i]^4-4\E[X_i]^3\E[Y_i]+6\E[X_i]^2\E[Y_i]^2-4\E[X_i]\E[Y_i]^3+\E[Y_i]^4
\end{align}
which leads us to a variance of 
\begin{align}
    \Var[Z_i]&=\E[Z_i^2]-\E[Z_i]^2
    \\
    &=\E[X_i^2]^2+4\E[X_i^2]\E[Y_i^2]+\E[Y_i^2]^2-\E[X_i^4]-\E[Y_i^4]
    \\
    &\quad -4\E[X_i]\E[Y_i]\left(\E[X_i]\E[Y_i]+\E[X_i^2]+\E[Y_i]^2-\E[X_i]^2-\E[Y_i^2]\right)
    \\
    &=\E[X_i^2]^2+4\E[X_i^2]\E[Y_i^2]+\E[Y_i^2]^2-\E[X_i^4]-\E[Y_i^4]
    \\
    &\quad -4\E[X_i]\E[Y_i]\left(\E[X_i]\E[Y_i]+\Var[X_i]+\Var[Y_i]\right)
    \\
    &\leq 2(\E[X_i^2]+\E[Y_i^2])^2
\end{align}

We can now bound the variance {\color{red} can we use independence between the coordinates due to poissonization? The number of hits a specific $abc$ gets should be independent, no?}
\begin{equation}
    \Var[Z]=\sum_{b\in S,a,c}\Var[Z_{abc}]\leq 2\sum_{b\in S,a,c}(p_{ac|b}+q_{ac|b})^2M^4p_b^4\leq 6(\|p[S]\|_2^2+\|q[S]\|_2^2)M^2
\end{equation}
Poissonization guarantees that the number of times we see the index $abc$ and $a'b'c'$ are independent. This implies that the frequency at which we see pairs from different $b$'s is also different. However, for a fixed $b$, there is a correlation between seeing $b$'s. Seeing $(abc)$ from $X$ means we see $(abc)$ requires us to witness $(abc)$ first, then any other element from $b$, which can then not contribute to the next pair.
\begin{align}
    &\sum_{(a,c)}\sum_{(a',c')\neq (a,c)}\E[(Z_{abc}-\E[Z_{abc}])(Z_{a'bc'}-\E[Z_{a'bc'}])]
    \\
    &=\sum_{(a,c)}\sum_{(a',c')\neq (a,c)}\E[Z_{abc}Z_{a'bc'}]-\E[Z_{abc}]\E[Z_{a'bc'}]
    \\
    &\leq \sum_{(a,c)}\sum_{(a',c')\neq (a,c)}\E[Z_{abc}Z_{a'bc'}]
\end{align}
We note that 
\begin{align}
&(X_iX_i'-2X_iY_i+Y_iY_i')(X_jX_j'-2X_jY_j+Y_jY_j')
\\
&=X_iX_i'X_jX_j'-2X_iX_i'X_jY_j+X_iX_i'Y_jY_j'-2X_iY_iX_jX_j'+4X_iY_iX_jY_j-2X_iY_iY_jY_j'
\\
&\quad +Y_iY_i'X_jX_j'-2Y_iY_i'X_jY_j+Y_iY_i'Y_jY_j'
\end{align}
expectation value:
\begin{align}
&\E[(X_iX_i'-2X_iY_i+Y_iY_i')(X_jX_j'-2X_jY_j+Y_jY_j')]
\\
&=(\E[X_iX_j])^2-2\E[X_iX_j]\E[Y_j]E[X_i]+(\E[X_iY_j])^2-2\E[X_iX_j]\E[Y_i]\E[X_j]+4\E[X_iX_j]\E[Y_iY_j]
\\&\quad -2\E[Y_iY_j]\E[X_i]\E[Y_j]+(\E[Y_iX_j])^2-2\E[Y_iY_j]\E[X_j]\E[Y_i]+(\E[Y_iY_j])^2
\end{align}
and summing up gives 
\begin{align}
&\sum_{i,j}(\E[X_iX_j])^2-4(\E[X_iX_j]+\E[Y_iY_j])\E[Y_j]\E[X_i]+2\E[X_i]^2\E[Y_j]^2+4\E[X_iX_j]\E[Y_iY_j]
+(\E[Y_iY_j])^2
\\
&\leq 2 \sum_{i,j}(\E[X_iX_j]+\E[Y_iY_j])^2+2\E[X_i]^2\E[Y_j]^2
\end{align}

Using the fact that $(x+y)^2 \leq 2(x^2+y^2)$, we finally find a covariance of 
\begin{align}4\sum_{(a,b,c)}\sum_{(a',b,c')\setminus (a,b,c)}\E[X_{abc}X_{a'bc'}]^2+\E[Y_{abc}Y_{a'bc'}]^2+2\E[X_{abc}]^2\E[Y_{a'bc'}]^2
\end{align}

Such that 
\begin{align}
    \sum_b\sum_{(a,c)}\sum_{(a',c')\setminus (a,c)}\E[X_{abc}X_{a'bc'}]^2&\leq \sum_b\sum_{(a,c)}\sum_{(a',c')}p_{ac|b}^2p_{a'c'|b}^2p_b^6M^6
    \\
    &\leq \sum_b\sum_{(a,c)}p_{abc}^2p_b^4M^6
    \\
    &\leq \|p[S]\|_2^2M^2,
\end{align}
and analogously for the term $\E[Y_{abc}Y_{a'bc'}]^2$.
Next, we want to bound 
\begin{align}
    \sum_b\sum_{(a,c)}\sum_{(a',c')\setminus (a,c)}\E[X_{abc}]^2\E[Y_{a'bc'}]^2&\leq \sum_{(a,c)}\sum_{(a',c')} p_{ac|b}^2(p_{a'|b}p_{c'|b})^2M^8p_b^8\\
    &\leq \sum_{(a,c)} p_{ac|b}^2M^8p_b^8\leq \|p[S]\|_2^2M^2
\end{align}
So the covariance is in $O(\|p[S]\|_2^2M^2)$, just like $\sum_b\Var[Z_b]$.
\end{proof}

and 

and our estimator will be 
\begin{align}
    Z=\sum_{abc}Z_{abc},\quad Z_{abc}:=X_{abc}X'_{abc}-2X_{abc}Y_{abc}+Y_{abc}Y'_{abc}.
\end{align}
We will calculate $\E[Z]$ and $\Var[Z]$, which we expand in $x$. We will also argue that this expansion is valid. 
We now want to bound the expectation value and the variance of this estimator. For readability we write $i$ instead of $abc$. Then, for a specific index $i$,
\begin{align}
    \E[Z_i]&=\E[X_i]\E[X'_i]-2\E[X_i]\E[Y_i]+\E[Y_i]\E[Y_i']
    =\left(\E[X_i]-\E[Y_i]\right)^2
\end{align}
Assume wlog $p_{ac|b}>q_{ac|b}$ (otherwise flip the roles of $p$ and $q$). We next use $e^{-x}\geq 1-x+x^2/4$. This holds because $f(0):=e^{-0}=g(0):=1-0+0^2/4$, and for the first derivative, we have that $f'(x)=-e^{-x}\geq g(x)-1+x/2$, which holds for $x<1$. Then
\begin{align}
    \E[X_{abc}]-\E[Y_{abc}]&=(p_{ac|b}-q_{ac|b})\left[\frac{Mp_b}{2}-\frac{1}{2}\sinh(Mp_b)e^{-Mp_b}\right]
    \\
    &=(p_{ac|b}-q_{ac|b})\left[\frac{Mp_b}{2}-\frac{1}{4}+\frac{1}{4}e^{-2Mp_b}\right]
    \\
    &\geq\frac{p_{ac|b}-q_{ac|b}}{4}M^2p_b^2
\end{align}
So we get 
\begin{equation}
    \E[Z]=\sum_{abc}\frac{(p_{ac|b}-q_{ac|b})^2}{16}M^4p_b^4\geq \frac{M^4\epsilon^2}{64d_B^2}\|p_{abc}-q_{abc}\|_2^2
\end{equation}
To lower bound the farness case, we use the known fact that $D_H^2(p,q)\leq \sqrt{d\|p-q\|_2^2}$ CHECK, and since we have a lower bound on $D_H^2(p,q)\geq \epsilon$, we can bound 
\begin{equation}
    \E[Z]\geq \frac{M^4\epsilon^4}{c d_Ad_B^3d_C}.
\end{equation}
Next we bound the variance. For simplicity, write again $i:=abc$. We will need:

For both $p$ and $q$, we can bound
\begin{equation}
    \|p[S]\|_2^2\leq \sum_{abc\in S}p_{ac|b}^2p_b^2\leq \sum_{b\in S}p_b^2 \leq \min\{1/M,d_B/M^2\}
\end{equation}
such that 
\begin{equation}
    \Var[Z]\leq 12\min\{M, d_B\}.
\end{equation}
We want to apply the Chebyshev inequality, and set the threshold at the middle between $0$ and $\E[Z]$, so at $M^4\epsilon^4/2cd_Ad_B^3d_C$. To apply Chebyshev, we then need 
\begin{equation}
    \sqrt{\Var[Z]}\ll \frac{M^4\epsilon^4}{2cd_Ad_B^3d_C}.
\end{equation}
Dependent on the two cases and ignoring constants, this implies
\begin{equation}
    \frac{M^4\epsilon^4}{d_Ad_B^3d_C}\geq d_B^{1/2}\implies M\geq \frac{d_A^{1/4}d_B^{7/8}d_C^{1/4}}{\epsilon},\quad\quad\frac{M^4\epsilon^4}{d_Ad_B^3d_C}\geq M^{1/2}\implies M\geq \frac{d_A^{2/7}d_B^{6/7}d_C^{2/7}}{\epsilon^{8/7}}. 
\end{equation}


\subsubsection{OLD}
We first want to lower bound the number of $b$'s we expect to collide when taking $N$ samples. For simplicity (and since we only want a lower bound), consider only $b$'s for which $p_b\leq o(1/N)$. We will bound the probability that such a $b$ appears at least twice by the opposite event:

\begin{subequations}
\begin{align}
    \Pr[\# b <2]&=(1-p_b)^N+p_b(1-p_b)^{N-1}\binom{N}{1}\\
    &\leq (1-p_b+Np_b)(1-p_b)^{N-1}\\
    &\leq (1+(N-1)p_b)\left(1-(N-1)p_b +(N-1)^2p_b^2/2 +O\left((p_bN)^3\right)\right)\\
    &\leq 1-(N-1)^2p_b^2+(N-1)^2p_b^2/2+O\left((Np_b)^3\right)\\
    &\leq 1-(N-1)^2p_b^2/2+O\left((Np_b)^3\right).
\end{align}
\end{subequations}
Hence, the probability to see a $b$ at least twice if $p_b\leq o(1/N)$ is still in $\Theta(N^2p_b^2)$. For larger $p_b$'s, in $\Theta(1/N)$, we get a probability in $\theta(1)$, which we can also bound by $\Theta(N^2p_b^2)$. Together, we conclude that the expected number of $b$'s from $S$ which we see at least twice can be lower bounded by 
\begin{equation}
    \Omega\left(\sum_{b\in S}N^2p_b^2\right)=\Omega\left(N^2\|p[S]\|_2^2\right).
\end{equation}
With the Markov inequality applied to both $X$ as the number of $b$'s we see more than twice, and $\bar{X}$, we see that the actual value is within a constant factor of the actual one with high probability.

Unlike the $b$'s in $L$, where each has its own bin, we just create one large bin for all small $b$'s, $B_S$: for each of the $O(N^2\|p[S]\|_2^2)$ pairs which collided, we pick two samples, say $(a,b,c)$ and $(a',b,c')$ (there might be more!) and add $(a,b,c')$ to the bin. {\color{red} Not sure whether this is fine with dependencies and everything!}
When we now sample in the second stage and draw a sample with $b\in S$, we ignore that sample, and instead return a random sample from $B_S$. As mentioned, we do not actually sample from $p_{AB}p_{BC}/p_B$ with this technique - but we will argue that the damage we inflict to the value of $D_H^2$ is relatively minor. Importantly, we also need to sample a bit different from $p$ as well, to ensure the two distributions coincide if $p_{ABC}=p_{AB}p_{BC}/p_B$. This is achieved by also first taking $N$ samples: we don't create bins for the large ones, but create a large bin for $S$. If we have collisions, we just pick a random sample for each of the colliding small $b$'s.
In the second stage, we draw $n$ samples: if it is large, we return it, if it is small, we discard it and return a random sample from $B_S$ instead. {\color{red}drawing from a finite bin will cause some dependencies, so I expect that we will need Poissonization or something?}


We have the probability for a $S$ to appear changes as follows (ignoring constant factors):
\begin{equation}
    p_b\rightarrow \frac{(\sum_{b'\in S}p_{b'})(p_bN)^2}{\sum_{b'\in S}(p_{b'}N)^2}=\frac{|p[S]|p_b^2}{\|p[S]\|_2^2}, 
\end{equation}
{\color{red}Need to argue that $p_{ac|B=b}$ does not change in our new way of sampling (and same for the reference distribution).}
Since we intend to replace it later with the mutual information, we introduce
\begin{equation}
    J(A:C|B=b)_{p}:=
    \begin{cases}
        \sum_{a,c}\left(\sqrt{p_{ac|B=b}}-\sqrt{p_{a|B=b}p_{c|B=b}}\right)^2 & \text{if }p_b>0,\\
        0 &\text{else.}
    \end{cases}
\end{equation}
Note that 
\begin{equation}
    \frac{\tilde p_{abc}}{\tilde p_b}=\frac{\frac{|p[S]|}{\|p[S]\|_2^2}\frac{p_{abc}}{p[S]}}{\frac{|p[S]|}{\|p[S]\|_2^2}\frac{p_{b}}{p[S]}}=\frac{p_{abc}}{p_b},
\end{equation}
which implies that $J(A:C|B=b)_p=J(A:C|B=b)_{\tilde p}$. Also note that we can write
\begin{equation}
    D_H^2\left(p_{ABC}[S],\frac{p_{AB}p_{BC}}{p_B}[S]\right)=\sum_{b\in S}\sum_{a,c}\left(\sqrt{p_{abc}}-\sqrt{p_{ab}p_{bc}/p_b}\right)^2=\sum_{b\in S}p_bJ(A:C|B=b)_p.
\end{equation}
Our quantity of interest changes as follows:
\begin{equation}
    J(A:C|B)_{ p}=\sum_{b\in S}p_bJ(A:C|B=b)_{p}\quad \rightarrow \quad \E[J(A:C|B)_{\tilde  p}]=\E\left[\sum_{b\in S}\tilde p_bJ(A:C|B=b)_{\tilde p}\right]
\end{equation}
here we bounded the thing by a coin toss
Now note that due to the Poissonization, we can treat the different $\tilde p_b$'s as independent. 
\begin{align}
    \E[\tilde p_b]&=\Pr[b\in N]\cdot \Pr[\text{sampled }b'\in S]\Pr[\text{sampled }b\in B_S]+\Pr[b\notin N]\cdot 0\\
    &\geq (p_bN)^2\cdot \frac{\left(\sum_{b\in S}p_b\right)}{\sum_{b\in S}(p_bN)^2}
    =\frac{|p[S]|p_b^2}{\|p[S]\|_2^2}, 
\end{align}
and we can say that (note we can ignore elements smaller $\epsilon/2d_B$)
\begin{equation}
    \E[J(A:C|B)_{\tilde p}]\geq \frac{|p[S]|p_b^{\min}}{\|p[S]\|_2^2}\sum_b p_bJ(A:C|B)_{\tilde p}\geq \frac{|p[S]|\epsilon}{2d_B\|p[S]\|_2^2}J(A:C|B)_p.
\end{equation}
We care about the probability that this is still close to the true value.
Using that there are no correlations due to the Poissonization trick ({\color{red}CHECK!})
\begin{align}
    \Var\left[\sum_{b\in S}p_bJ(A:C|B=b)_{p}\right]&=\sum_{b\in S}J(A:C|B=b)_{\tilde p}^2\Var[\tilde p_b]
    \\
    &\leq J_{\max}^2\sum_{b\in S}\E[\tilde p_b^2]
    \\
    &\leq J_{\max}^2\sum_{b\in S}(Np_b)^2\left(\frac{\left(\sum_{b\in S}p_b\right)}{\sum_{b\in S}(p_bN)^2}\right)^2\\
    &= J_{\max}^2\frac{\left(\sum_{b\in S}p_b\right)^2}{\sum_{b\in S}(p_bN)^2}\\
    &\leq \frac{J_{\max}^2d_B|p[S]|^2}{N^2\|p[S]\|_2^2},
\end{align}
which means that we are good for $N\geq O(J_{\max}\sqrt{d_B}/\epsilon)$, since we can then still reliable distinguish between (set $I(A:C|B)_p=\epsilon/2$ in ???)
\begin{equation}
    \frac{|p[S]|\epsilon^2}{4d_B\|p[S]\|_2^2}\quad\text{and}\quad 0
\end{equation}

so the mutual information is modified as 
\begin{align}
    D_H^2(p[S],q[S])=\sum_bp_b D_H^2(p[b],q[b])\rightarrow \sum_b \frac{|p[S]|p_b^2}{\|p[S]\|_2^2} D_H^2(p[b],q[b])&=\frac{|p[S]|p_b}{\|p[S]\|_2^2}D_H^2(p[S],q[S])\\
    &\geq \frac{|p[S]|\epsilon}{2d_B\|p[S]\|_2^2}D_H^2(p[S],q[S]),
\end{align}
since we argued that we can ignore $p_b<\epsilon/2d_B$.
If we take $N$ samples, we get the probability of a $b$ being in a collision is in $O(p_b^2N^2)$. As such, the number of collisions is expected to be at least $\sum_{b\in S}p_b^2N^2=\|p[S]\|_2^2N^2$. 
{\color{red} We might need to explicitly calculate $\|p[S]\|_2^2$, but I think that is possible: the lemma in the beginning of section 4 says that we can find $\tilde c$ with $l_2^2\leq \tilde c \leq (l_2+\eta)^2\leq 2l_2^2+\eta^2$ in $\sqrt{d}+1/\eta$. We know that $l_2$ needs to be at least $\epsilon^2/2d_B$ (CHECK!), so I think that should be fine, since we would set $\eta=\epsilon/\sqrt{d_B}$?}

We now want to use the equivalence tester on $S$. The distance between the two elements is reduced by the factor given above, but at the same time we need to renormalize it by a factor $1/p[S]$ (I think/hope), meaning we test for a gap $\eta=\epsilon\cdot \epsilon/2d_B\|p[S]\|_2^2$. We then need to choose $N$ such that there are certainly enough collisions:

So how many samples do we need? Recall there are two cases, the sample complexity is $\min{|S|^{3/4}/\eta,|S|^{2/3}/\eta^{4/3}}$ 
\begin{equation}
    \frac{|S|^{3/4}\|p[S]\|_2^2d_B}{\epsilon^2}\overset{!}\leq N^2\|p[S]\|_2^2\implies N\geq \frac{|S|^{3/8}d_B^{1/2}}{\epsilon},
\end{equation}
which we can achieve using $N\geq d_B^{7/8}/\epsilon$ many samples. {\color{red} I think this comes from the fact that the threshold, when which case is better, was shifted from MI to CMI.}

On the other hand, we can use $d_B^{2/3}/\epsilon^{4/3}$. Inserted, this gives 
\begin{equation}
    \frac{|S|^{2/3}(\|p[S]\|_2^2d_B)^{4/3}}{\epsilon^{8/3}}\overset{!}\leq N^2\|p[S]\|_2^2\implies N\geq (\|p[S]\|_2^2)^{1/6}\frac{d_B}{\epsilon^{4/3}}
\end{equation}
Note that
\begin{equation}
    \|p[S]\|_2^2\leq \min\{|S|/N^2,1/N\}.
\end{equation}
The first term comes from the fact that the maximal probability in $p[S]$ is $1/N$, and there are at most $|S|$ elements. The second term comes from the fact that $|S|/N$ has to be smaller than one, otherwise $|p[S]|>1$. Then we get two cases:
\begin{equation}
    N_1\geq (d_B/N_1^2)^{1/6}\frac{d_B}{\epsilon^{4/3}}\implies N_1\geq \frac{d_B^{7/8}}{\epsilon},
    \quad 
    N_2\geq (1/N_2)^{1/6}\frac{d_B}{\epsilon^{4/3}}\implies N_1\geq \frac{d_B^{6/7}}{\epsilon^{8/7}}.
\end{equation}
We can take either inequality, so the sample complexity is
\begin{equation}
    \tilde O\left(\min\left\{\frac{d_B^{7/8}}{\epsilon},\frac{d_B^{6/7}}{\epsilon^{8/7}}\right\}\right),
\end{equation}
and by Canonne, this is tight. The edge case is when $d_B=N$, implying that $d_B^{1/8}=1/\epsilon$.

\subsubsection{Considering $d_A$ and $d_C$ as Well}
(Back of an envelope quality for now.) We again have 
\begin{equation}
    \frac{|S_{ABC}|^{2/3}(\|p_B[S]\|_2^2d_B)^{4/3}}{\epsilon^{8/3}}\overset{!}\leq N^2\|p_B[S]\|_2^2\implies N\geq (\|p[S]\|_2^2)^{1/6}\frac{d_A^{1/3}d_Bd_C^{1/3}}{\epsilon^{4/3}} ,
\end{equation}
and with $\|p_B[S]\|_2^2\leq \min\{|S_B|/N^2,1/N\}$, we get
\begin{align}
    N_1&\geq (d_B/N_1^2)^{1/6}\frac{d_A^{1/3}d_Bd_C^{1/3}}{\epsilon^{4/3}}\implies N_1\geq \frac{d_A^{1/4}d_B^{7/8}d_C^{1/4}}{\epsilon},
    \\ 
    N_2&\geq (1/N_2)^{1/6}\frac{d_A^{1/3}d_Bd_C^{1/3}}{\epsilon^{4/3}}\implies N_2\geq \frac{d_A^{2/7}d_B^{6/7}d_C^{2/7}}{\epsilon^{8/7}}.
\end{align}
Since we can choose either of the two bounds $N_1$ or $N_2$, we end up with 
\begin{equation}
    N_S=O\left(\min\left\{\frac{d_A^{1/4}d_B^{7/8}d_C^{1/4}}{\epsilon},\frac{d_A^{2/7}d_B^{6/7}d_C^{2/7}}{\epsilon^{8/7}}\right\}\right).
\end{equation}

\subsubsection{Large Eigenvalues}
(Note: log factors are missing in certain places, eg make a Chernoff bound to make sure something is valid for all parameters etc...)
\begin{proof}
    In the first step of the algorithm, we considered $b$'s with very small eigenvalues: the remaining $b$'s are such that $p_b$ is bounded from below, and we know it up to a constant/log factor. The basic idea will be a binning in two steps: for each $b$ we bin the values $(a,c)$ according to the values of $p_{a|b}$ and $p_{c|b}$ on a grid. Then we bin similar $b$'s together. In the end, we will have split the distribution into a polylogarithmic number of categories $\{S^{ij}_k\}$, which we will test using \cref{lemma:equivalence_l2} using $N$ samples each. To create these samples from the reference distribution $p_{ab}p_{bc}/p_b$, we perform two stages. First, we take $\tilde O(N)$ samples which we sort according to their $b$-value into queues. In the second round we take the exact amount of samples we need, say $\tilde N$. If we draw $(a,b,c)$, we go to bin $b$ and pick a random sample with the same $b$-value, $(a',b,c')$, and we return $(a,b,c')$. Since small $b$'s are excluded, concentration bounds guarantee us that with high probability, the queues from the first round contain enough samples for the second round. (Note that \cref{lemma:equivalence_l2} works using samples directly from $p$ and $q$).
    
    We first want to empirically estimate the probability distribution $p_{a|b}:=p_{ab}/p_b$. For a specific $b$, we will see $Np_b$ many samples, which allows us to determine all $p_{a|b}$ larger than $1/Np_b$ up to a constant/$\log$ factor, and we split them into $O(\log(N))$ (actually $O(\log(Np_b))$) many bins. All smaller values are put into a separate bin. 
    \begin{itemize}
        \item Let $K_b$ be one of the large bins for a fixed $b$. Then, whp., for all $a,a'\in K$ satisfy that $1/2\log(N)\leq p_{a|b}/p_{a'|b}\leq 2\log(N)$.
        \item For each $b$, the last bin contains all $a$ such that $p_{a|b}\leq 1/Np_b$, or equivalently $p_{ab}\leq 1/N$, without lower bound.
    \end{itemize}
    For each $b$, we then do the same for $C$ with different $\log(N)$ bins using $O(N)$ new samples. The assumption that the number of samples gives us this can be checked using Chernoff.
    
    {\color{blue} OLD. Let $A_i$ be the random variable indicating how often index $i$ was observed. Note that by adjusting the implicit constant accordingly, we have that for all bins, except the last one, $\E[A_i]=N p_i\geq 10\log^4(N)/uv$. {\color{blue}{Note: this already guarantees a constant factor, no?}} Then
    \begin{equation}
        \Pr[|A_i-\E[A_i]|\geq \E[A_i]/2]\leq e^{-\E[A_i]/10}\leq e^{-\log(N)/uv}\leq \frac{\epsilon}{d_Ad_C}.
    \end{equation}
    With a union bound, this holds for all $A$ and $C$ together.

    For the smallest bin, we use a different formulation of Chernoff, namely $\Pr[X\geq (1+\delta)\E[X]]\leq e^{-\delta^2\E[X]/(2+\delta)}$ for $\delta> 0$. We pick $\delta$ such that $\delta \E[X]=3\delta Np_i=3\log(N)$. Then, 
    \begin{equation}
        \Pr[A_i\geq \log(N)]\leq e^{-\log(N)}
    \end{equation}
    is small as well.
}
For a specific $b$ we now have two sets of bins, $\{A_i^{b}\}_i$ sorting the $a$ values depending on $p_{a|b}$ and $\{C_i^{b}\}_i$ sorting the $c$ values depending on $p_{c|b}$. We can form a two dimensional grid of categories $S^b_{ij}:=A_i^b\times C_j^b$, the set of which we denote by $\mathcal{S}$, $\mathcal{S}^b:=\{S^b_{i,j}\}_{i,j}$. 

Next, we will group $b$'s with similar $p_b$ together, which we know up to a log-factor anyways. There are $k_b:=\log(1/p_b^{\min})=O(\log(d_B/\epsilon))$ many bins, $B_k$. Recall that all $p_b$ are bounded from below! We can then combine the categories of all the $b$'s contained in a $B_k$, $S_{i,j}^{B_k}:=\cup_{b\in B_k}S_{i,j}^{b}$.


Further, for a category $S$, let $S_A=\{a~|~\exists c: (a,c)\in S\}$, and $S_C$ analogously. Note that $|S|\leq |S_A||S_C|$\footnote{Note that we do not need $|S|=|S_A||S_C|$}. We can also write 

Since all $p_b$ are the same up to a constant afctor, we also have that for all $i,j$, all $b,b'\in B_k$ and $(a,c)\in S_{ij}^b$ and $(a',c')\in S_{ij}^{b'}$ that $p_{ab}/p_{a'b'}=\Theta(1)$, $p_{ab}/p_{a'b'}=\Theta(1)$. This allows us to write
    \begin{align}
        D_H^2(p,q)&=\sum_bp_b\sum_{(a,c)}\left(\sqrt{\frac{p_{abc}}{p_b}}-\sqrt{\frac{p_{ab}}{p_b}\frac{p_{bc}}{p_b}}\right)^2\\
        &= \sum_{k=1}^{k_b}\sum_{i,j}\sum_{b\in B_k}\sum_{(a,c)\in S_{ij}^{b}}p_b\left(\sqrt{\frac{p_{abc}}{p_b}}-\sqrt{\frac{p_{ab}}{p_b}\frac{p_{bc}}{p_b}}\right)^2\\
        &\leq\sum_{k=1}^{k_b}\sum_{i,j}\underbrace{\sum_{b\in B_k}\sum_{(a,c)\in S_{ij}^{b}}\max_{b\in B_k}\{p_b\}\left(\sqrt{\frac{p_{abc}}{p_b}}-\sqrt{\frac{p_{ab}}{p_b}\frac{p_{bc}}{p_b}}\right)^2}_{z_{i,j}^k}.
    \end{align}
    This means in particular that if $D_H^2(p,q)\geq \epsilon$, then by the pigeonhole principle, at least one of the $O(\log(\log(N)^2\log(d_B/\epsilon)))$ categories $z_{i,j}^k$ needs to satisfy $z_{i,j}^k\geq \epsilon/\log^3(N)$ ({\color{red}considering $p_b$, a $\log^2$ might be enough?}). We will test this individually for each $z_{i,j}^k$. Depending on whether $S$ contains a last bin or not, we need to apply different approaches.
    \begin{itemize}    
        \item \textbf{Heavy categories:}
        This includes all categories where neither $a$ nor $c$ come from the last bin, such that for all $a,b,c$ both $p_{a|b}$ an $p_{c|b}$ are bounded away from zero. We can bound 
        \begin{align}
        \label{eq:dh_indep:heavy_bound}
            z_{i,j}^k&
            =\sum_{b\in B_k}\sum_{(a,c)\in S_{ij}^{b}}\max_{b\in B_k}\{p_b\}\left(\sqrt{\frac{p_{abc}}{p_b}}-\sqrt{\frac{p_{ab}}{p_b}\frac{p_{bc}}{p_b}}\right)^2
            \\
            &=\max_{b\in B_k}\{p_b\}|B_i|\sum_{b\in B_k}\sum_{(a,c)\in S_{ij}^{b}}\frac{\left(\frac{p_{abc}}{|B_k|p_b}-\frac{p_{ab}p_{bc}}{|B_k|p_b^2}\right)^2}{\left(\sqrt{\frac{p_{abc}}{|B_k|p_b}}+\sqrt{\frac{p_{ab}p_{bc}}{|B_k|p_b^2}}\right)^2}\\
            &\leq 4|B_k|\frac{\max_{b\in B_k}\{p_b\}}{\max_{\substack{b\in B_k \\(a,c)\in S_{ij}^{b}}}\{p_{ab}p_{bc}/p_b^2|B_k|\}}\|p_{B_k}[S_{ij}^{b}]-q_{B_k}[S_{ij}^{b}]\|_2^2,
        \end{align}
        where we introduced  $p_{B_i}(a,b,c):=p_{abc}/|B_i|p_b$ ($q$ analogously), which forms a probability distribution over $S^{B_k}_{ij}$, hence the notation. Thus, testing whether $z_{i,S}=0\text{ vs }z_{i,S}\geq \epsilon/\log^3(m)$ can be solved by distinguishing
        \begin{equation}
            p_{B_k}[S_{ij}^{B_k}]=q_{B_k}[S_{ij}^{B_k}]\quad\text{vs}\quad\|p_{B_k}[S_{ij}^{B_k}]-q_{B_k}[S_{ij}^{B_k}]\|_2\geq O(\eta),
        \end{equation}
        where 
        \begin{equation}\eta:=\sqrt{\frac{  \epsilon \max\limits_{b\in B_k,(a,c)\in S_{ij}^{b}}\left\{\frac{p_{ab}p_{bc}}{p_b^2}\right\}}{\log^3(m)|B_k|^2\max_{b\in B_k}\{p_b\}}}.
        \end{equation}
        Equivalence testing for $l_2$ wrt $\eta$ costs $O(\|q_{B_k}[S_{ij}^{B_k}]\|_2/\eta^2)$ samples. Note that 
        \begin{equation}
        \label{eq:dh_indep:l_2_norm}
            \|q_{B_k}[S_{ij}^{B_k}]\|_2\leq \frac{1}{|B_k|}\sqrt{\sum_{b\in B_k}\sum_{(a,c)\in S_{ij}^{b}}\left(\frac{p_{ab}p_{bc}}{p_b^2}\right)^2}\leq \sqrt{\frac{|S_{ij}^{B_k}|}{|B_k|}}\max_{b\in B_k,(a,c)\in S_{ij}^{b}}\left\{\frac{p_{ab}p_{bc}}{p_b^2}\right\}.
        \end{equation}
        Hence, the sample complexity of solving our decision problem is \begin{align}
            O\left(\log^3(m)\sqrt{|S_{ij}^{B_k}||B_i|^3}\max_{b\in B_i}\{p_b\}/\epsilon\right)
        \end{align} 
        many samples from $B_i$. Taking $N$ samples, we get $O(N|B_i|\max_{b\in B_i}\{p_b\})$ many samples from $B_i$. Solving for $N$ gives us
        \begin{equation}
            N\geq O\left(\log^3(m)\sqrt{|S_{ij}^{B_k}||B_i|}/\epsilon\right).
        \end{equation}
        Then $N\geq O\left(\log^3(m)\sqrt{d_Ad_Bd_C}/\epsilon\right)$ would be enough.
        \item \textbf{Mixed categories:}
        (In the following, we fix the indices $i,j,k$ implicitly, and simply write $S$ instead of $S_{ij}^{B_k}$ when the context is clear). We would again like to upper bound $D_H^2(p[S],q[S])$ by $\|p[S]-q[S]\|_2$. This time however, it is a bit more complicated, as the trick from \eqref{eq:dh_indep:heavy_bound} doesn't work anymore: there is no lower bound on $q_i$. Assume without loss of generality that the unbounded coordinate comes from $A$, i.e.\ $p_{a|b}\leq 1/Np_b$. Instead, we denote by $S_-$ the set of indices in $S$ for which $(\sqrt{p_{abc}}-\sqrt{p_{ab}p_{bc}/p_b})^2/|B_i|p_b\leq x$, for $x\in (0,1)$ to be determined, and $S_+:=S\setminus S_-$. Note that for indices in $S_+$, we have $x<p_{ab}p_{bc}/|B_k|p_b^2$ Then 
        \begin{align}
            &D_H^2(p[S],q[S])
            \\
            &= \sum_{b\in B_k}p_b|B_k|\left[\sum_{(a,c)\in S_+}\left(\sqrt{\frac{p_{abc}}{|B_k|p_b}}-\sqrt{\frac{p_{ab}p_{bc}}{|B_k|p_b^2}}\right)^2+
            \sum_{(a,c)\in S_-}\left(\sqrt{\frac{p_{abc}}{|B_k|p_b}}-\sqrt{\frac{p_{ab}p_{bc}}{|B_k|p_b^2}}\right)^2\right]\\
            &\leq \sum_{b\in B_k}p_b|B_k|\sum_{(a,c)\in S_+}\frac{1}{x}\left(\frac{p_{abc}}{|B_k|p_b}-\frac{p_{ab}p_{bc}}{|B_k|p_b^2}\right)^2+1[p[S]\neq q[S]]\sum_{b\in B_k}p_b|B_k||S_-|x\\
            &\leq \frac{\max_{b\in B_k}\{p_b\}|B_k|}{x}\|p_{B_k}[S]-q_{B_k}[S]\|_2^2+1[p[S]\neq q[S]]\max_{b\in B_k}\{p_b\}|B_k|^2|S|x,
        \end{align}
        such that, for $x$ small enough,
        \begin{align}
            &\frac{\epsilon}{\log^2(m)}\leq D_H^2(p[S],q[S])
            \\
            &\implies \sqrt{\frac{x\epsilon}{\max_{b\in B_k}\{p_b\}\log^2(m)|B_k|}-|B_k||S|x^2}\leq \|p[S]-q[S]\|_2.
        \end{align}
        We want the first term under the square root to dominate the second one, which implies that we need to set 
        \begin{equation}
            x\leq O\left(\frac{\epsilon}{\max_{b\in B_k}\{p_b\}\log^2(m)|B_k|^2|S|}\right).
        \end{equation}
        As a result, we need to solve the decision problem of whether 
        \begin{equation}
            \|p[S]-q[S]\|_2\geq \tilde\epsilon:=\frac{\epsilon}{\max_{b\in B_k}\{p_b\}|B_k|^{3/2}|S|^{1/2}}\quad \text{or}\quad p=q.
            \label{eq:cmi_upper:eps}
        \end{equation}
        There are two ways to bound $\|q[S]\|_2$:
        \begin{align}
            \|q[S]\|_2=\sqrt{\sum_{b\in B_k,(a,c)\in S}\left(\frac{p_{ab}p_{bc}}{|B_k|p_b^2}\right)^2}\leq 
            \begin{cases} 
                \sqrt{|S||B_k|}\max_{b\in B_k,(a,c)\in S}\left\{\frac{p_{ab}p_{bc}}{|B_k|p_b^2}\right\} &\text{(Case 1)}
            \\
                \sqrt{\max_{b\in B_k,(a,c)\in S}\left\{\frac{p_{ab}p_{bc}}{|B_k|p_b^2}\right\}} 
                &\text{(Case 2)}
            \end{cases}
            \label{eq:cmi_upper:l2}
        \end{align}
        We can further use that $p_{bc}/p_b\leq O(1/|S_C|)$, since all $p_{bc}/p_b$ are the same up to a constant, and $\sum_{c\in S_C}p_{bc}/p_b$ is upper bounded by $1$. We know from Lemma \ref{???} That $\|q[S]\|_2/\tilde\epsilon^2$ samples of $p|_{B_i}$ will be needed: from $N$ samples, $Np_b|B_k|$ will have the right value. Then
        \begin{align}
            \text{Case 1:}\quad\frac{\|q[S]\|_2}{\tilde \epsilon^2}&\leq \frac{\sqrt{|S|/|B_k|}\max_{b\in B_k,(a,c)\in S}\{q_{ab}q_{bc}/q_b^2\}}{\tilde \epsilon^2}\\
            &\leq \frac{|S_A|^{1/2}\max_{b\in B_k,(a,c)\in S}\{q_{ab}/q_b\}}{\tilde \epsilon^2|S_B|^{1/2}|S_C|^{1/2}}\\
            (A\text{ small})\quad &\leq \frac{|S_A|^{1/2}}{\tilde \epsilon^2 |B_k|^{1/2}|S_C|^{1/2} N p_b}\\
            &\leq \frac{|S_A|^{3/2}|B_k|^{5/2}|S_C|^{1/2}p_b}{ \epsilon^2  N}\overset{!}=Np_b|B_k|,\\
            \implies N&\geq \frac{|S_A|^{3/4}|B_k|^{3/4}|S_C|^{1/4}}{ \epsilon}
            \\
            \text{Case 2:}\quad\frac{\|q[S]\|_2}{\tilde \epsilon^2}&\leq \frac{\sqrt{\max_{b\in B_k,(a,c)\in S}\{q_{ab}q_{bc}/q_b^2\}/|B_k|}}{\tilde \epsilon^2}\\
            &\leq \frac{1}{\tilde \epsilon^2\sqrt{|B_k||S_C|Np_b}}\\
            &\leq \frac{p_b^2|B_k|^3|S|}{ \epsilon^2\sqrt{|B_k||S_C|Np_b}}\\
            &\leq \frac{p_b^{3/2}|B_k|^{5/2}|S_A||S_C|^{1/2}}{\epsilon^2\sqrt{N}}\overset{!}= Np_b|B_i|\\
            \implies N &\geq \frac{p_b^{1/3}|B_k||S_A|^{2/3}|S_C|^{1/3}}{\epsilon^{4/3}},
        \end{align}
        which we can ensure by picking $p_B|B_i|\leq 1$ (note that the two cases are still different, because we dont have sum over $b$'s alone, but also $S$), resulting in
        \begin{equation}
            N \geq \frac{|B_k|^{2/3}|S_A|^{2/3}|S_C|^{1/3}}{\epsilon^{4/3}}.
        \end{equation}
        We then need to do the same for the case where the roles of $A$ and $C$ are switched. Assuming $d_A\geq d_C$, this results in a sample complexity of 
        \begin{equation}
            N\geq O\left(\min\left\{\frac{d_A^{3/4}d_B^{3/4}d_C^{1/4}}{\epsilon},\frac{d_A^{2/3}d_B^{2/3}d_C^{1/3}}{\epsilon^{4/3}}\right\}\right)
        \end{equation}
        \item \textbf{Light category:}
        There is one category where both $a$ and $c$ are light. The previous argument works analogously for the most part, but note that we can no longer use $p_{bc}/p_b\leq O(1/|S_C|)$: before we could argue that $\sum_cp_{bc}/p_b\leq 1$, and all terms are equal up to a constant factor, which doesn't work anymore. As such, we need to use other ways to bound the sample complexity, $\|q[S]\|_2/\tilde\epsilon^2$. Note however that we can still take the values for $\tilde\epsilon$ from \eqref{eq:cmi_upper:eps} and $\|q[S]\|_2$ from \eqref{eq:cmi_upper:l2}). Using Case 2 with $p_{ab}/p_b,p_{bc}/p_b\leq 1/N$:
        \begin{align}
            \frac{\sqrt{\max_{b\in B_k,(a,c)\in S}\{q_{ab}q_{bc}/q_b^2\}/|B_k|}}{\tilde \epsilon^2}
            &\leq\frac{\sqrt{p_{ab}p_{bc}/p_b^2|B_k|}p_b^2|B_k|^3|S|}{\epsilon^2}
            \\
            &\leq \frac{|B_k|^{5/2}|S|p_b^2}{\epsilon^2Np_b}\overset{!}\leq Np_b|B_k|
            \\
            \implies N&\geq \frac{|B_k|^{3/4}|S|^{1/2}}{\epsilon}.
        \end{align}
        Note that Case 1 gives a result which is strictly worse, namely 
        \begin{align}
            \frac{\sqrt{|S|/|B_i|}p_b^2|B_i|^3|S|p_{ab}p_{bc}/p_b^2}{\epsilon^2}&\leq \frac{|B_i|^{5/2}|S|^{3/2}p_b^2}{\epsilon^2N^2p_b^2}\overset{!}=Np_b|B_i|\implies N\geq \frac{|B_i|^{1/2}|S|^{1/2}}{\epsilon^{2/3}p_b^{1/3}}.
        \end{align}
        Inserting the values for $p_b$ derived in ???: $p_b\geq \epsilon/d_B^{7/8}$ we obtain $N\geq |S|^{1/2}d_B^{19/24}/\epsilon$ and $p_b\geq \epsilon^{8/7}/d_B^{6/7}$ gives $N\geq |S|^{1/2}d_B^{11/14}/\epsilon^{22/21}$. Considering also $d_A$, $d_C$ makes matters worse. 
    \end{itemize}
    Combining both regimes give us
    \begin{equation}
    O\left(\max\left\{\min\left\{\frac{d_A^{3/4}d_B^{3/4}d_C^{1/4}}{\epsilon},\frac{d_A^{2/3}d_B^{2/3}d_C^{1/3}}{\epsilon^{4/3}}\right\},\frac{d_A^{1/2}d_B^{3/4}d_C^{1/2}}{\epsilon},\min\left\{\frac{d_A^{1/4}d_B^{7/8}d_C^{1/4}}{\epsilon},\frac{d_A^{2/7}d_B^{6/7}d_C^{2/7}}{\epsilon^{8/7}}\right\}\right\}\right).
\end{equation}
\end{proof}



\begin{figure}[H]
        \begin{center}

\begin{tikzpicture}

\def\binX{0.25}
\def\binY{0.5}
\def\tcol{blue}

\draw[->] (-0.1,-0.6) -- (5,-0.6);
\draw[->] (-0.1,-0.6) -- (3.5-0.1,3.5-0.6);
\draw[dashed] (0.5,0.05) -- (5.5,0.05);
\draw[dashed] (-0.1+1.1,-0.6) -- (3.5-0.1+1.1,3.5-0.6);
\foreach \j in {0,...,3}{
\foreach \i in {3,...,0}
{
    \def\sc{1}
    \def\spx{1.2*\j+\binX*\i + 0.375*\i}
    \def\spy{2.5*\binX*\i}

    \tkzDefPoint(\spx,\spy){A} 
    \tkzDefPoint(\spx,\spy-0.5){Al} 
    
    \tkzDefPoint(\spx+1,\spy){B} 
    \tkzDefPoint(\spx+1,\spy-0.5){Bl} 
    \tkzDefPoint(\spx+1.5,\spy+0.5){C} 
    \tkzDefPoint(\spx+1.5,\spy+0.5-0.5){Cl} 
    \tkzDefPointWith[colinear= at C](B,A) \tkzGetPoint{D}
    \ifthenelse{\i = 0}{
        \ifthenelse{\j = 0}{\def\tcol{red}}{\def\tcol{purple}}
    }{
        \ifthenelse{\j = 0}{\def\tcol{purple}}{\def\tcol{blue}}
    } 
    \tkzDrawPolygon[fill=\tcol!10](A,B,C,D)
    \tkzDrawPolygon[fill=\tcol!10](Al,A,B,Bl)
    \tkzDrawPolygon[fill=\tcol!10](Bl,B,C,Cl)
}
}

    \def\spx{3}
    \def\spy{3.5}
    \tkzDefPoint(\spx,\spy){A} 
    \tkzDefPoint(\spx,\spy-0.5){Al} 
    
    \tkzDefPoint(\spx+1,\spy){B} 
    \tkzDefPoint(\spx+1,\spy-0.5){Bl} 
    \tkzDefPoint(\spx+1.5,\spy+0.5){C} 
    \tkzDefPoint(\spx+1.5,\spy+0.5-0.5){Cl} 
    \tkzDefPointWith[colinear= at C](B,A) \tkzGetPoint{D}
    \tkzDrawPolygon[fill=\tcol!10](A,B,C,D)
    \tkzDrawPolygon[fill=\tcol!10](Al,A,B,Bl)
    \tkzDrawPolygon[fill=\tcol!10](Bl,B,C,Cl)

\node at (1, -1) {$p_{abc}$};

\end{tikzpicture}
\caption{\label{bla}We could make the outermost line of boxes of larger size to show that it might be larger dependent on $b$.}
    \end{center}
\end{figure}
